A Study of Lagrangean Decompositions and Dual Ascent Solvers for Graph Matching

We study the quadratic assignment problem, in computer vision also known as graph matching. Two leading solvers for this problem optimize the Lagrange decomposition duals with sub-gradient and dual ascent (also known as message passing) updates. We explore s direction further and propose several additional Lagrangean relaxations of the graph matching problem along with corresponding algorithms, which are all based on a common dual ascent framework. Our extensive empirical evaluation gives several theoretical insights and suggests a new state-of-the-art any-time solver for the considered problem. Our improvement over state-of-the-art is particularly visible on a new dataset with large-scale sparse problem instances containing more than 500 graph nodes each.

==> abstract-mp.tex <==
\section{Abstract Message Passing}
\label{sec:AbstractMessagePassing}

\paragraph{Energy Minimization as ILP.} 
Let $I:=\sum_{i\in\SV}|\SX_i| + \sum_{ij\in\SE}|\SE|$ be the total number of all values of the potentials. We will denote by $\theta\in
\BR^{I}$ the vector with coordinates $(\theta_i(x_i)\colon i\in\SV,\ x_i\in\SX_i)$ and $(\theta_{ij}(x_{ij})\colon ij\in\SE,\ x_{ij}\in\SX_{ij})$.
Problem~\eqref{eq:energy-min} can be formulated as an integer linear program (ILP) (see e.g.~\cite{Werner07})
\begin{align}\label{eq:ILP:objective}
 & \min\nolimits_{\mu_i\in\BR_+^{|\SX_i|},\ i\in\SV \atop 
                  \mu_{ij}\in\BR_+^{|\SX_{ij}|},\ j\in\SE}\langle \theta,\mu\rangle  \\
&\mbox{s.t.}\  
\left\{
\begin{array}{lll}
  i\in\SV, & \sum_{x_i\in\SX_i} \mu_i(x_i) = 1,\\
  ij\in\SE, & \sum_{x_{ij}\in\SX_{ij}} \mu_{ij}(x_{ij}) = 1,\\
  ij\in\SE,\  x_i\in\SX_i, & \sum_{x_j\in\SX_j} \mu_{ij}(x_{ij}) = \mu_{i}(x_i), \\
  ij\in\SE,\  x_j\in\SX_j, & \sum_{x_i\in\SX_i} \mu_{ij}(x_{ij}) = \mu_{j}(x_j),\quad
\end{array} \vline\ 
\begin{array}{lll}
   A_i\mu_i=b_i\\
   A_{ij}\mu_{ij}=b_{ij}\\
   A_{(ij,i)}\mu_{ij}=A_{(i,ij)}\mu_i \\
   A_{(ij,j)}\mu_{ij}=A_{(j,ij)}\mu_j 
\end{array} 
\right. \label{eq:ILP:linear-constraints}
\\ \label{eq:ILP:integrality-constraints}
 &\mu \in \{0,1\}^I
\end{align}
{\color{red} Comment about an additional constraint}
Omitting the integrality constraints~\eqref{eq:ILP:integrality-constraints} one obtains the {\em local polytope relaxation}, denoted by $\Lambda_{\SG}$, of the energy minimization problem~\eqref{eq:energy-min}.
It can be seen, that linear constraints~\eqref{eq:ILP:linear-constraints} have a separable form, which is explicitly written to the right of the vertical line for suitably selected matrices $A_i$, $A_{ij}$, $A_{(i,ij)}$, $A_{(j,ji)}$, $A_{(ij,i)}$ $A_{(ij,j)}$.
In what follows we consider a general class of such separable problems.

\paragraph{Pairwise-Separable Linear Programs (IPS-LP).}
% general LP formulation (10), getting back to energy minimization as an example
% additional general linear constraints fit to the format, e.g. assignment - eq.(9), point out the main example-graph-matching - in Section XXX
Linear problems (LP) of the form
\begin{align}
\label{eq:FactorLP}
&\min_{\mu_1 \in \R_+^{d_1},\ldots,\mu_k \in \R_+^{d_k}} \sum_{i \in BV} \la\theta_i,\mu_i\ra\\ \nonumber
&\text{s.t.} 
\begin{cases}
 A_i \mu_i = b_i,&  i \in \BV \\
 A_{(i,j)} \mu_i = A_{(j,i)} \mu_j, & ij \in \BE\subset \{ ij: i\neq j\}
\end{cases}
\end{align}
%will be called {\em pairwise-separable}. Furthermore, we will assume that 
will be called {\em pairwise-separable}. Furthermore, if 
\begin{itemize}
 \item the extreme points of $\{\mu_i \geq 0\ :\ A_i \mu_i = b_i\}$ are a subset of $\{0,1\}^{d_i}$;
 \item $A_{(i,j)},A_{(j,i)}$ are $\{0,1\}$-matrices such that for a suitable integer $K$ it holds\\
$\left\{A_{(i,j)} \mu_i :  \mu_i \in \{0,1\}^{d_i}, A_i \mu_i = b_i \right\} \in \{0,1\}^{K}$
 and likewise for $A_{(j,i)} \mu_j$,
\end{itemize}
we will call~\eqref{eq:FactorLP} {\em integer-relaxed} and use the acronym IPS-LP for this class of integer-relaxed pairwise-separable problems.
The pair $\BG = (\BV,\BE)$ will be called \emph{factor graph}.
To each factor $i \in \BF$ we associate the tuple $(A_i,b_i)$ defining the corresponding \emph{coupling constraints} of the factor.
To each edge $ij \in \BE$ we associate the tuple $(A_{(i,j)}, A_{(j,i)})$ defining the coupling constraints.
As one can see from~\eqref{eq:ILP:objective}-\eqref{eq:ILP:linear-constraints}, the local polytope relaxation of the energy minimization problem~\eqref{eq:energy-min} can be represented as IPS-LP as follows.
Let the factors be $\BV = \SV \cup \SE$, i.e. the factors correspond to the \emph{unary marginals} $\mu_i$, $i \in \SV$ and to the \emph{pariwise marginals} $\mu_{ij}$, $ij \in \SE$ in the local polytope relaxation~\eqref{eq:ILP:objective}-\eqref{eq:ILP:linear-constraints}.
The nodes of the factor graph are hence the nodes \emph{and} edges of the original graphical model.
The edges $\BE$ of the factor graph correspond to pairs $(i,ij)$, $ij \in \SE$.
%Different binary vectors $\mu_k$ in~\eqref{eq:FactorLP} correspond to \emph{unary} $\mu_i$ and \emph{pairwise marginals} $\mu_{ij}$ in the local polytope relaxation~\eqref{eq:ILP:objective}-\eqref{eq:ILP:linear-constraints}. This generalizes also to graphical models with higher order factors~\cite{Werner10}, i.e.\ those including potentials depending on three and more variables. There, a separate binary vector would correspond also to each such factor. Therefore we will use the term {\em factors} for the variables $\mu_i$, $i=1,\dots,k$ from~\eqref{eq:FactorLP} and denote {\color{red} the set of such variables as $\BV=\{???\}$}. 
% what is the formal definition of the set? Set of indices or better the set of vector spaces? Or \BV=\{d_i, i=\overline{1,k}\}
%The set $\BE\subset \{ ij: i\neq j\}$ introduced in~\eqref{eq:FactorLP} denotes neighborhoods of the factors. Two factors $\mu_i\in ?$ and $\mu_j$ are {\em neighboring} if there is a constraint $A_{(i,j)} \mu_i = A_{(j,i)} \mu_j$ in~\eqref{eq:FactorLP}. In what followsd these constraints will be called {\em coupling} and the pair $(\BV,\BE)=:\BG$ a {\em factor graph}.

\paragraph{Linear Constraints in IPS-LP}

{\color{red} Consider the problem~\eqref{eq:energy-min} and an additional linear constraint. Show how it fits into the IPS-LP format}

\paragraph{Dual IPS-LP}.
The dual problem to~\eqref{eq:FactorLP} reads 
\begin{align}
\label{eq:DualFactorLP}
\max_{z,\phi} &  \sum_{i=1}^k \la b_i, z_i\ra \\ \nonumber
\text{s.t.} &  
\begin{cases}
A_i^\T z_i \leq  \theta^{\phi}_i := \theta_i + \sum_{j \in \SN_{G}(i)} A_{(i,j)}^\T \phi_{(i,j)},\ i=\overline{1,k}  \\
\phi_{(i,j)}=-\phi_{(j,i)},\ ij\in F\,.
\end{cases}
\end{align}
We provide its derivation in the supplementary material.
Compare~\eqref{eq:DualFactorLP} to the dual for the {\color{red} plain} energy minimization~\eqref{eq:ILP:objective}-\eqref{eq:ILP:linear-constraints}
%, where $\SE(i):=\{i\in\SV\colon ij\in\SE\}$ denotes all edges incident to the node $i$:
\begin{align}
\label{eq:energy-dual-LP}
\max_{z,\phi} & \sum_{i=1}^k \la \eins, z_i\ra\\ \nonumber
\mbox{s.t.} &
\begin{cases}
z_i \leq  \theta^{\phi}_i(x_i) := \theta_i(x_i) + \sum_{ij \in \SN(i)_{\SG}} \phi_{(i,ij)}(x_i), i\in\SV,\ x_i\in\SX_i \\
z_{ij} \leq  \theta_{ij}^{\phi}(x_{ij}): = \theta_{ij}(x_{ij})-\phi_{(i,ij)}(x_i)-\phi_{(j,ij)}(x_j), ij\in\SE,\ x_{ij}\in\SX_{ij}  
\end{cases}
\end{align}
The plain LP dual~\eqref{eq:energy-dual-LP} contains only messages $\phi_{(i,ij)}$ directed from unary to pairwise {\color{red} factors}. The general dual problem~\eqref{eq:DualFactorLP} also can be formulated only with the directed messages $\phi_{(i,j)}$ such that $i < j$. We introduced however also "reverse" messages $\phi_{(j,i)}:=-\phi_{(i,j)}$ for $j>i$ to simplify the notation. Introducing such additional "reverse" messages would only turn the last inequality in~\eqref{eq:energy-dual-LP} into  
$z_{ij} \leq  \theta_{ij}^{\phi}(x_{ij}): = \theta_{ij}(x_{ij})+\phi_{(ij,i)}(x_i)+\phi_{(ij,j)}(x_j)$. 

In the sequel we implicitly assume the constraint $\phi_{(i,j)}=-\phi_{(j,i)},\ ij\in F$ to hold, if not stated otherwise.

The modified costs $\theta^{\phi}$ from~\eqref{eq:DualFactorLP} are called \emph{reparametrizations} of the potentials~$\theta$.
In the supplementary we provide the proof that $\sum_{i} \la \theta_i,\mu_i\ra = \sum_{i} \la \theta^{\phi}_i,\mu_i\ra$, whenever $\mu_1,\ldots,\mu_k$ are feasible for the coupling constraints.
%For fixed dual variables $\phi$ from~\eqref{eq:DualFactorLP}, we can compute the~\emph{dual lower bound} as follows.
Duality theory implies that any fixed messages $\phi$ from~\eqref{eq:DualFactorLP} determine the lower bound 
\begin{equation}
\label{eq:DualLowerBound}
L(\phi) := \sum_{i=1}^k \max_{z_i} \{ \la b_i, z_i \ra : A_i^\T z_i \leq \theta^{\phi}_i\}
\end{equation}
for the optimum of~\eqref{eq:FactorLP}. The function $L$ is concave in $\phi$, as we prove in the supplement. 

\textcolor{red}{$\phi'_{(i,j)}$ denotes a message difference. Better denote it by $\Delta_{(i,j)}$ or by some other notation yet?}

\paragraph{Abstract Message Passing: Dual Block-Coordinate Ascent for IPS-LP}
% Abstract Dual, compare to the local polytope dual 
% Block-Coordinate Updates, its variants: SRMP, MP-LP, MSD
% Lemma 1
% Block-Coordinate Ascent Algorithm
% Thm. 1; Weak convergence, in special cases - arc consistency in the limit
% 
% \begin{algorithm}
% \label{alg:MessagePassingUpdate}
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \Input{Factor $i\in\BV$, subset $J = \{j_1,\ldots,j_l\} \subseteq \SN_{\BG}(i)$ of neigboring factors, current dual variables $\phi$}
% Compute locally optimal factor values:
% \begin{equation}
% \label{eq:FactorOptimization}
% \mu_i^* \in \argmin\nolimits_{\mu_i \in\BR_{+}^{d_i}} \la \theta^{\phi}_i, \mu_i \ra \quad \text{s.t. } A_i \mu_i = b_i
% \end{equation}
% \\
% Choose $\delta \in \R^{d_i}$ s.t. $\delta(j) \left\{ \begin{array}{ll} > 0, & \mu^*_i(j) > 0 \\ < 0,& \mu^*_i(j) = 0 \end{array} \right.$,\quad  e.g. $\delta=\left\{ \begin{array}{rl}1, & \mu^*_i(j) > 0 \\ -1,& \mu^*_i(j) = 0 \end{array}\right.$\,.\\
% Compute messages to the neighboring factors from $J$:
% \begin{equation}
% \label{eq:ReverseFactorOptimization}
% \begin{array}{lcl}
% \begin{pmatrix}\phi^*_{(i,j_1)}, \ldots, \phi^*_{(i,j_l)} \end{pmatrix} \in &
% \argmax\limits_{\phi'_{(i,j_1)},\ldots,\phi'_{(i,j_l)}} 
% & \sum_{j \in J} \la \delta, \theta_i^{\phi} - \sum_{j \in J} A^\T_{(i,j)} \phi'_{(i,j)} \ra \\
% &\text{s.t.}& \mu_i^* \in \argmin\limits_{\mu_i \geq 0: A_i \mu_i = b_i} \la \mu_i,\theta^{\phi}_i - \sum_{j \in J} A^\T_{(i,j)} \phi'_{(i,j)} \ra \\ 
% & & \la e_c, \phi'_{(i,j)} \ra \leq 0 \quad \forall \la e_c, (A_{(i,j)} \mu_i) \ra = 0 \\
% & & \la e_c, \phi'_{(i,j)} \ra \geq 0 \quad \forall \la e_c, (A_{(i,j)} \mu_i) \ra = 1 \\
% \end{array}
% \end{equation}\\
% \Output{$\phi*_{(i,j)}$ $\forall j \in J$.}
% \caption{Message-Passing Update Step}
% \end{algorithm}

\begin{algorithm}
\label{alg:MessagePassingUpdate}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Factor $i\in\BV$, subset $J = \{j_1,\ldots,j_l\} \subseteq \SN_{\BG}(i)$ of neigboring factors, current dual variables $\phi$}
Compute locally optimal factor values:
\begin{equation}
\label{eq:FactorOptimization}
\mu_i^* \in \argmin\limits_{\mu_i} \la \theta^{\phi}_i, \mu_i \ra \quad \text{s.t. }  \mu_i\ge 0,\  A_i \mu_i = b_i
\end{equation}
\\
Choose $\delta \in \R^{d_i}$ s.t. $\delta(s) \left\{ \begin{array}{ll} < 0, & \mu^*_i(s) > 0 \\ > 0,& \mu^*_i(s) = 0 \end{array} \right.$,\quad  e.g. $\delta(s)=\left\{ \begin{array}{rl} -1, & \mu^*_i(s) > 0 \\ 1,& \mu^*_i(s) = 0 \end{array}\right.$\,.\\

Define $\theta_i^{\phi+\phi'}:=\theta_i^{\phi}+\sum_{j \in J} A^\T_{(i,j)} \phi'_{(i,j)}$.\\
Compute messages to the neighboring factors from $J$:
\begin{equation}
\label{eq:ReverseFactorOptimization}
\begin{array}{lcl}
\begin{pmatrix}\phi^*_{(i,j_1)}, \ldots, \phi^*_{(i,j_l)} \end{pmatrix} \in &
\argmax\limits_{\phi'_{(i,j_1)},\ldots,\phi'_{(i,j_l)}} 
& \sum_{j \in J} \la \delta,\theta_i^{\phi+\phi'} \ra \\
&\text{s.t.}& \mu_i^* \in\hspace{-1pt} \argmin\limits_{\mu_i\ge 0: A_i \mu_i = b_i} \la \mu_i,\theta_i^{\phi+\phi'} \ra \\ 
& & \phi'_{(i,j)}(s) 
\begin{cases}
\le 0, & \nu_i(s) =0\\
\ge 0, & \nu_i(s) =1
\end{cases},
\text{where}\ \nu_i:=A_{(i,j)} \mu^*_i
% & & \la e_c, \phi'_{(i,j)} \ra \leq 0 \quad \forall \la e_c, (A_{(i,j)} \mu^*_i) \ra = 0 \\
% & & \la e_c, \phi'_{(i,j)} \ra \geq 0 \quad \forall \la e_c, (A_{(i,j)} \mu^*_i) \ra = 1 \\
\end{array}
\end{equation}\\
\Output{$\phi^*_{(i,j)}$ $\forall j \in J$.}
\caption{Message-Passing Update Step. }
\end{algorithm}

The dual bound $L(\phi)$~\eqref{eq:DualLowerBound} only depends on messages $\phi$, not on $z$. 
To maximize $L$, we will iteratively visit all factors and adjust messages $\phi$ connected to it, such as to achieve a monotonically increasing sequence of messages.

% local update: only variable and some of its neighbours
% feasible: small LP - one factor - in (9)
% Small LP (1 factor + some neighbors), sine the first constraint can be written as a set of linear constraints, hm... its size grows exponentially with d_i
First, we present the elementary message update step in Algorithm~\ref{alg:MessagePassingUpdate}.
In words, Algorithm~\ref{alg:MessagePassingUpdate} does the following: 
Given a factor $i$ and a subset subset $J$ of neigboring factors, 
we first compute the locally optimal value of the primal $\mu_i$, without the coupling constraints. For the plain energy minimization~\eqref{eq:ILP:objective}-\eqref{eq:ILP:linear-constraints} it would mean selecting the factor state with the smallest value of the reparametrized potential $\theta^{\phi}_i$. 
Then we set up $\delta$ so, that the potentials $\theta^{\phi+\phi'}_i:=\theta^{\phi}_i + \sum_{j \in J} A^\T_{(i,j)}$ will tend to increase for locally optimal {\color{red}states} $s$ (where $\mu_i(s)>0$) and to decrease for locally non-optimal ones. However, during these changes, 
the locally optimal states $s$ must remain locally optimal, according to the first constraint in~\eqref{eq:ReverseFactorOptimization}. 
{\color{red} The last two conditions in~\eqref{eq:ReverseFactorOptimization} are required to ...}
Overall, we basically push the slack from the factor $i$ in the inequality $A_i^T z_i \leq \theta_i^{\phi}$ to the factors $j \in J$.


% Then we choose a dual objective $\delta$ which is positive, whenever an entry of $\mu_i$ is so, and negative otherwise.
% Third, we make the reparametrized costs via dual variables $\phi'$ maximally unfavourable to current solution $\mu_i^*$ w.r.t. $\delta$ under the constraint that $\mu_i^*$ is still optimal to the new reparametrization
% $\theta^{\phi} - \sum_{j \in J} A^\T_{(i,j)} \phi'_{(i,j)}$.
% The reweighting by $\omega$ will ensure overall convergence when we perform multiple such message passing updates simultaneously.
% Heuristically, this means that we push slack from factor $i$ in the inequality $A_i^T z_i \leq \theta_i^{\phi}$ to factors $j \in J$.
% 
% First, we present the elementary message update step in Algorithm~\ref{alg:MessagePassingUpdate}.
% In words, Algorithm~\ref{alg:MessagePassingUpdate} does the following: 
% Given a factor $i$ and a subset of connected messages $\phi_{(i,j)}, j \in J \subseteq \SN_F(i)$, 
% we first compute the optimal value of the primal $\mu_i$ without the coupling constraints.
% Then we choose a dual objective $\delta$ which is positive, whenever an entry of $\mu_i$ is so, and negative otherwise.
% Third, we make the reparametrized costs via dual variables $\phi'$ maximally unfavourable to current solution $\mu_i^*$ w.r.t. $\delta$ under the constraint that $\mu_i^*$ is still optimal to the new reparametrization
% $\theta^{\phi} - \sum_{j \in J} A^\T_{(i,j)} \phi'_{(i,j)}$.
% The reweighting by $\omega$ will ensure overall convergence when we perform multiple such message passing updates simultaneously.
% Heuristically, this means that we push slack from factor $i$ in the inequality $A_i^T z_i \leq \theta_i^{\phi}$ to factors $j \in J$.
%
The following lemma will be used to identify monotonicity of our message passing algorithm.
\begin{lemma}
\label{lemma:MessagePassingUpdateIncrease}
Let $\phi^*_{(i,j)}$, $j\in J$ be computed by Algorithm~\ref{alg:MessagePassingUpdate} for given $i\in\BV$,~$J$ and~$\phi$. Let 
$\tilde\phi(i',j')=
\begin{cases} 
\phi(i',j'),  & i'\neq i\ \text{or}\ j'\notin J \\ 
\phi(i',j')+\omega\phi^*_{(i',j')}, & \text{otherwise}
\end{cases}$

Then $L(\tilde\phi) \ge L(\phi)$ whenever $\omega \in [0,1]$.
\end{lemma}
% \begin{proof}
% Let $\mu_j^* \in \argmin_{\mu_j \geq 0: A_j \mu_j = b_j} \la \theta^{\phi}_j,\mu_j \ra$ be an integral solution of~\eqref{eq:FactorOptimization} at which the dual lower bound~\eqref{eq:DualLowerBound} is attained before the update
% and $\mu'_j \in \argmin_{\mu_j \geq 0: A_j \mu_j = b_j} \la \theta^{\phi} + A_{(j,i)}^\T \phi'_{(i,j)}, \mu_j \ra$ be an integral solution at which the dual lower bound is attained after $\phi$ has been updated.
% Note that $\mu_i^* = \mu'_i$ can be chosen.
% We need to prove 
% \begin{equation}
% \la \theta^{\phi}_i,\mu_i^*\ra + \sum_{j \in J} \la \theta^{\phi}_j, \mu_j^*\ra \leq \la \theta^{\phi}_i - \sum_{j \in J} A^\T_{(i,j)} \phi'_{(i,j)} ,\mu'_i\ra + \sum_{j \in J} \la \theta^{\phi}_j + A^\T_{(j,i)} \phi'_{(i,j)} , \mu'_j\ra \,.
% \end{equation}
% We shuffle all terms with variables $\phi_{(i,j)}$, $j \in J$ to the right side and all other terms to the left side.
% \begin{equation}
% \la \theta_i^{\phi}, \mu^*_i - \mu'_i \ra + \sum_{j \in J} \la \theta_j^{\phi}, \mu^*_j - \mu'_j \ra \leq \la \sum_{j \in } -A^\T_{(i,j)} \phi_{(i,j)}, \mu'_i \ra + \sum_{j \in J} \la A^\T_{(j,i)} \phi_{(i,j)}, \mu'_j \ra
% \end{equation}
% The leftmost term cancels out due to $\mu^*_i = \mu'_i$. All other terms on the left side are smaller than zero due to the choice of $\mu^*_j$ being minimizers w.r.t. $\theta^{\phi}_j$.
% Hence, it will be enough to prove the above inequality when assuming the left side to be zero.
% We rewrite the scalar products by transposing $A^\T_{(i,j)}$ and $A^\T_{(j,i)}$. 
% \begin{equation}
% %0 \leq \sum_{j \in J} \left\{\la \phi_{(i,j)}, A_{(j,i)} x'_j \ra + \la \phi_{(i,j)}, - A_{(i,j)} x_i^* \ra \right\}
% 0 \leq \sum_{j \in J} \left\{\la \phi_{(i,j)}, A_{(j,i)} \mu'_j - A_{(i,j)} \mu_i^* \ra \right\}
% \end{equation}
% Due to $A_{(j,i)} \mu'_j \in \{0,1\}^{\dim(\phi_{(i,j)})}$ and $A_{(i,j)} \mu_i^* \in \{0,1\}^{\dim(\phi_{(i,j)})}$ by assumption and $\phi_{(i,j)} \lessgtr 0$ whenever $A_{(i,j)} \mu^*_i \lessgtr 0$, the result follows.
% Also scaling with $\omega$ will decrease the lower bound $L$ from~\eqref{eq:DualLowerBound}, as it is convex.
% \end{proof}

Finally, we combine message passing updates in Algorithm~\ref{alg:AbstractMessagePassing}.

\begin{algorithm}
\label{alg:AbstractMessagePassing}
\For{$i=1,\ldots,k$ in some order} {
\textbf{Receive Messages:}\\
\For{$j \neq i$} {
Compute new $\phi^*_{(j,i)}$ with $\omega=1$ and $J = \{j\}$ by Algorithm~\ref{alg:MessagePassingUpdate}. \\
Set $\phi_{(j,i)} = \phi_{(j,i)} - \phi^*_{(j,i)}$. \\
}
\textbf{Round Primal Solution:}\\
Compute $\mu_i^* \in \argmin_{\mu_i \geq 0} \la \theta^{\phi},\mu_i \ra \quad \text{s.t. } A_i \mu_i = b_i, A_{(i,j)} \mu_i = A_{(j,i)} \mu_j^*$ $\forall \mu_j^*$ already visited.\\
\textbf{Send Messages:}\\
Choose Partition $J_1 \dot{\cup} \ldots \dot{\cup} J_l = \SN_{G}(i)$.\\
Choose weights $\omega_{J_1},\ldots,\omega_{J_l} \geq 0$ such that $ \omega_{J_1} + \ldots \omega_{J_l} \leq 1$.\\
\For{$J \in \{J_1,\ldots,J_s\}$} {
Compute new $\phi^*_{(i,j)}$ for $J$ with weights $\omega_{J}$ by Algorithm~\ref{alg:MessagePassingUpdate}.
}
\For{$J \in \{J_1,\ldots,J_l\}$} {
Set $\phi_{(i,j)} = \phi_{(i,j)} - \omega_{J} \phi^*_{(i,j)}$ $\forall j \in J$.
}
}
\caption{One Iteration of Message-Passing}
\end{algorithm}

Algorithm~\ref{alg:AbstractMessagePassing} works as follows: It visits the nodes of the factor graph in some order. First, it receives messages from all connected factors, minimizing the slack in all connected factor. Then, we round a primal solution for the visited factor such that it is consistent w.r.t. the coupling constraints with the previously obtained primal solution of the connected factors.
Finally, we send messages to all connected factors, minimizing the slack in the current factor. Reweighting by $\omega$ has to be done to ensure monotonical convergence.
We choose weights $\omega$ similarly as in~\cite{SRMPKolmogorov} and choose a-priori a factor order, which we traverse alternatingly in forward and backward direction, as also done in~\cite{SRMPKolmogorov}.

\begin{theorem}
Algorithm~\ref{alg:AbstractMessagePassing} is monotonically increasing the dual lower bound.
\end{theorem}
\begin{proof}
We need to proof that (i) the receiving messages step and (ii) the sending messages step improve the dual lower bound~\eqref{eq:DualLowerBound}.

\noindent(i) Directly apply Lemma~\ref{lemma:MessagePassingUpdateIncrease}.
(ii) The difficulty here is that we compute descent directions from the current dual variables $\phi$ in parallel and then apply all of them simultaneously. 
The dual lower bound $L(\phi)$ is convex,  hence we apply Jensen's inequality to obtain the result.

\end{proof}
It can be seen that Algorithm~\ref{alg:AbstractMessagePassing} subsumes known message-passing algorithms like MSD~\cite{Werner07}, TRW-S~\cite{TRWSKolmogorov}, SRMP~\cite{SRMPKolmogorov} and MPLP~\cite{MPLP}.


==> graph-matching.tex <==
\section{Graph Matching}
\label{sec:GraphMatching}
We will apply our abstract message-passing framework from Section~\ref{sec:AbstractMessagePassing} to the graph matching problem.
To this end, we will present three general approaches expressible as IPS-LPs to the graph matching problem and apply it to the original graph matching problem, an inverse formulation of the graph matching problem and one that combines both.

\paragraph{Graphical Model, Factors}
We consider the MAP-inference problem~\eqref{eq:energy-min} with the special label set $\SX_i \subseteq \SV$, i.e. the set of potential labels corresponds to a subset of nodes of the graph $\SG$.
The graph matching problem is
\begin{equation}
  \label{eq:GraphMatching}
  \min_{x \in \mathcal{X}_{\SV}} \sum_{i \in \SV} \theta_i(x_i) + \sum_{ij \in \SE} \theta_{ij}(x_{ij}) \quad \text{s.t. } x_i \neq x_j \ \forall i\neq j
\end{equation}
Figure~\ref{fig:ExampleGraphMatching} illustrates a small example.
\begin{wrapfigure}{L}{0.38\textwidth}
\begin{tikzpicture}
\tikzstyle{every node}=[draw,circle,fill=white,minimum size=6pt,inner sep=1pt]
\draw (0,1) node (i) {i};
\draw (0,0) node (j) {j};
\draw (1,0.5) node (k) {k};
\draw (i) -- node[rectangle](ij) {ij} (j) ;
\draw (i) -- node[rectangle](ik) {ik} (k) ;
\draw (j) -- node[rectangle](jk) {jk} (k) ;


\draw (3,1) node (i') {i'};
\draw (2.8,0) node (j') {j'};
\draw (3.5,0.1) node (k') {k'};


\path[->,thick,dashed,red,out=10,in=170] (i) edge (i');
\path[->,thick,dashed,red,out=-10,in=190] (j) edge (j');
\path[->,thick,dashed,red,out=5, in=150] (k) edge (k');
\end{tikzpicture}
\caption{
Exemplary graph matching problem.
Round nodes denote variables $\{i,j,k\} = \SV$, while rectangular nodes $\{ij,i,jk\} = \SE$ denote edges in the graphical model.
$\{i',j',l'\} = \SV'$ denote the nodes to be matched. Red dashed arrows signify the assignment.}
\label{fig:ExampleGraphMatching}
\end{wrapfigure}
The additional \emph{uniqueness constraint} means that each label may only be taken once.
Hence, a feasible labeling $x \in \SX$ corresponds to a permutation of $\SV$.
The graph matching problem~\eqref{eq:GraphMatching} can therefore also be approached in terms of the inverse permutation
To this end let the inverse graph $\SG' = (\SV',\SE')$ be given by $\SV' = \SV$, $\SE' = \left\{ ij\ :\ \exists x'_{ij} \in \SX'_{ij} \text{ s.t. } x'_i x'_j \in \SE \right\}$, the inverse label set $\mathcal{X}'_{\SV} = \prod_{i \in \SV} \mathcal{X}'_i$ with $\mathcal{X}'_i = \{j \in \SV : i \in \mathcal{X}_j\}$ and the inverse costs
\begin{equation}
%\begin{split}
\theta'_i(x'_i) = \theta_{x_i}(i),
\quad
\theta'_{ij}(x'_{ij}) = 
\left\{ \begin{array}{ll} 
\theta_{x'_{ij}}(i,j), & x'_{ij} \in \SE \\
0, & \text{ otherwise}
\end{array} \right.
%\end{split}
\end{equation}
Consider the resulting \emph{inverse graph matching} problem
\begin{equation}
  \label{eq:InverseGraphMatching}
  \min_{x' \in \mathcal{X}'_{\SV}} \sum_{i \in \SV} \theta'_i(x'_i) + \sum_{ij \in \SE} \theta'_{ij}(x'_{ij}) \quad \text{s.t. } x'_i \neq x'_j\  \forall i\neq j
%\sum_{i \in \SV} \theta_{x'_i}(i) + \sum_{ij \in \SE} \theta_{x'_{ij}}(i,j) \quad \text{s.t. } x'_i \neq x'_j\  \forall i\neq j
\end{equation}
Labeling $x \in \SX$ and inverse labeling $x' \in \SX'$ correspond to each other iff $x_{x'_i} = i$.

\begin{remark}
We also allow occlucion, i.e. we also may introduce a single extra label $\diamond$ which can be taken arbitrarly often.
This results in a partial matching, where the subset of variables $i \in \SV$ is matched for which $x_i \neq \diamond$.
We do not treat this case for simplicity of exposition.
\end{remark}

\paragraph{Encoding with Pairwise Potentials}
We add pairwise potentials and set the diagonals to $\infty$, i.e.
%\begin{equation}
$\theta_{ij}(x,x) = \infty$.
%\end{equation}
Any solution with cost $< \infty$ will be an assignment.
The resulting optimization problem is over the usual local polytope~\eqref{eq:ILP:linear-constraints}.

\paragraph{Coupling with the Inverse Problem}
We consider~\eqref{eq:GraphMatching} and~\eqref{eq:InverseGraphMatching} simultaneously.
Relaxing in terms of the local polytope relaxation~\eqref{eq:ILP:linear-constraints} leads to
\begin{equation}
\label{eq:UnaryInverseUnaryConstraint}
\min_{\mu \in \Lambda_{\SG},\mu' \in \Lambda_{\SG'}} \frac{1}{2} \left( \la \theta, \mu \ra + \la \theta', \mu' \ra \right) \quad \text{s.t.} \quad \mu_i(x_i) = \mu'_{x_i}(i)\  \forall i \in \SV, x_i \in \SX_i\,.
\end{equation}
The uniqueness constraint in~\eqref{eq:UnaryInverseUnaryConstraint} corresponds to $x_{x'_i} = i$.
The dual is
\begin{equation}
\label{eq:DualUnaryInverseUnaryConstraint}
\begin{array}{lll}
\max_{z,\phi} & \sum_{i \in \SV \dot{\cup} \SV'} z_i + \sum_{ij \in \SE \dot{\cup} \SE'} z_{ij} \\
\text{s.t.}
& z_{i} \leq \theta_i(x_i) + \sum_{ j \in \SN_{\SG \dot{\cup} \SG'}(i)} \phi_{(i,ij)}(x_i) + \boxed{\phi_{(i,x_i)}} & \forall i \in \SV \dot{\cup} \SV'\\
& z_{ij} \leq \theta_{ij}(x_{ij}) + \phi_{(ij,i)}(x_i) + \phi_{(ij,j)}(x_j) & \forall ij \in \SE \dot{\cup} \SE'\\
\end{array}
\end{equation}
The boxed variables in~\eqref{eq:DualUnaryInverseUnaryConstraint} indicate the additional dual variable corresponding to the constraint $\mu_i(x_i) = \mu'_i(x_i)$.
All other variables are present in the dual local polytope~\eqref{eq:ILP:linear-constraints}.

\begin{remark}
The constraint $\mu_i(x_i) = \mu'_{x_i}(i)$ in~\eqref{eq:UnaryInverseUnaryConstraint} could also be handled by a pairwise factor between 
$\mu_i$ and $\mu'_{x_i}$.
This would result in a standard pairwise graphical model.
However this approach requires $\dim(\mu_i) + \dim(\mu'_{x_i}$ dual variables and also simply running TRWS~\cite{TRWSKolmogorov} would result in suboptimal performance, as shown in the supplement.
\end{remark}

\paragraph{Encoding with a Linear Assignment Factor} 
Consider the auxiliary graph $\SG_{ass}=(\SV_{ass},\SE_{ass})$ consisting of the node set $\SV_{ass} = \{i:i \in\SV\} \dot{\cup} \{i':i' \in \SV'\}$ and the \emph{directed} edge set $\SE_{ass} = \{(i,j'): j \in \mathcal{X}_i\}$.
The edge set $\SE_{ass}$ corresponds to all possible labels in all nodes of the graph original problem~\eqref{eq:GraphMatching}.
The primal and dual assignment problem on $\SG_{ass}$ is
\begin{equation}
\label{eq:LinearAssignmentProblem}
\begin{array}{lr}
\min_{\mu_f} \langle \theta_{f}, \mu_f \rangle & \max_{\pi,\pi'} \la \eins, z_f \ra - \la \eins,z'_f \ra \\
\sum_{x_i : (i,x_i) \in \SE_{ass}} \mu_f(i,x_i) = 1 & z_f(i) \in \R   \\
- \sum_{i : (i,x_i) \in \SE_{ass}} \mu_f(i,x_i) = -1 & z'_f(x_i) \in \R \\
\mu_f(i,j') \geq 0 & -z_f(i) + z'_f(x_i) \leq \theta_f(i,x_i) \\
\end{array}
\end{equation}
In case $\mathcal{X}_i = \SV$ for $i \in \SV$, graph $\SG_{ass}$ is the full bipartite graph.
In either case, the resulting problem is a minimum cost flow problem and can be solved via efficient combinatorial solvers, see~\cite{AhujaMagnantiOrlinNetworkFlows} for an overview.
Denote the additional assignment factor with variables $\mu_f$ by $f$ and the constraint set for $\mu_f$ by $\Omega$.
The resulting problem is
\begin{equation}
\label{eq:FlowUnaryConstraint}
\min_{\mu \in \Lambda_{\SG}, \mu_f \in \Omega} \la \theta,\mu\ra \quad \text{s.t. } \mu_{i}(x_i) = \mu_{f}(i,x_i) \ \forall i\in\SV, x_i\in \SX_i\,.
\end{equation}
The dual to~\eqref{eq:FlowUnaryConstraint} (compare the $z_f$ and $z'_f$-variables to~\eqref{eq:LinearAssignmentProblem}) is
\begin{equation}
\label{eq:DualFlowUnaryConstraint}
\begin{array}{lll}
\max_{z,\phi} &\sum_{i \in \SV} z_i + \sum_{ij \in \SE} z_{ij} + \la \eins,z_f\ra - \la \eins, z'_f\ra \\
\text{s.t.}
& z_{i} \leq \theta_i(x_i) + \sum_{j \in \SN_{\SG}(i)} \phi_{(i,ij)}(x_i) + \boxed{ \phi_{(i,f)}(x_i) } & \forall i \in \SV\\
& z_{ij} \leq \theta_{ij}(x_{ij}) + \phi_{(ij,i)}(x_i) + \phi_{(ij,j)}(x_j) & \forall ij \in \SE\\
& \boxed{z_{f}(i) - z'_{f}(x_i) \leq \phi_{(f,i)}(x_i)} & \forall (i,x_i) \in \SE_{ass}\\
\end{array}
\end{equation}
The boxed variables correspond to the dual variables of the flow factor~\eqref{eq:LinearAssignmentProblem} and the coupling constraints linking them in~\eqref{eq:FlowUnaryConstraint}.
All other variables are present in the dual local polytope~\eqref{eq:ILP:linear-constraints}.

\section{Graph Matching Algorithms}
\label{sec:GraphMatchingAlgorithms}
Below we will present the optimization routines used inside Algorithm~\ref{alg:MessagePassingUpdate} for optimizing the graph matching problems~\eqref{eq:ILP:linear-constraints},~\eqref{eq:DualUnaryInverseUnaryConstraint} and~\eqref{eq:DualFlowUnaryConstraint}.
Specifically, Algorithm~\ref{alg:MessagePassingUpdate} requires solving~\eqref{eq:FactorOptimization} and~\eqref{eq:ReverseFactorOptimization}.
We will detail how to do this in the next two subsections.

\subsection{Obtaining an Optimal Factor Solution~\eqref{eq:FactorOptimization}}
When calling the message passing update Algorithm~\ref{alg:MessagePassingUpdate} for factor $i \in \BV$, we first have to find a locally optimal primal solution $\mu_i^*$ in~\eqref{eq:FactorOptimization}.
In all the studied problems we have only two kinds of factors: \emph{Simplex factors} $\{ \mu_i \geq 0: \la \eins,\mu_i \ra = 1\}$ and a linear assignment factor $\mu_f \in \Omega$. 
\paragraph{Simplex Factor}
For a simplex factor $\mu_i$ we can solve~\eqref{eq:FactorOptimization} by choosing a label $x_i^*\in \argmin_{x_i} \left\{ \theta_i^{\phi}(x_i) \right\}$.
\paragraph{Linear Assignment Factor}
For the linear assignment factor $\mu_f$ from~\eqref{eq:LinearAssignmentProblem} efficient minimum cost flow solvers exist, see~\cite{AhujaMagnantiOrlinNetworkFlows}.

\subsection{Solving the Reparametrization Adjustment Problem~\eqref{eq:ReverseFactorOptimization}}
After having found an optimal primal solution $\mu_i^*$ in~\eqref{eq:FactorOptimization} inside Algorithm~\ref{alg:MessagePassingUpdate}, we have to solve the reparametrization adjustment problem~\eqref{eq:ReverseFactorOptimization} corresponding to the coupling constraints $\phi_{(i,j)}$, $j \in J$.
In all our problems, there only exist the following coupling constraints and corresponding dual variables
(i)  between simplex factors $\mu_i, i \in \SV\dot{\cup}\SV'$ and $\mu_{ij}, ij \in \SE \dot{\cup} \SE'$ encoding unary-pairwise marginalization constraints present in~\eqref{eq:ILP:linear-constraints},
(ii) between two simplex factors $\mu_i, i \in \SV$ and $\mu_{i'}, i' \in \SV'$ encoding coupling~\eqref{eq:UnaryInverseUnaryConstraint} for the uniqueness constraint,
(iii) between a simplex factor $\mu_i, i \in \SV$ and the linear assignment factor $\mu_f$~\eqref{eq:LinearAssignmentProblem}. 
The corresponding messages are
(i) $\phi_{(i,ij)} = -\phi_{(ij,i)}$
(ii) $\phi_{(i,i')} = - \phi_{(i',i)}$
(iii) $\phi_{(i,f)} = -\phi_{(f,i)}$.

\paragraph{Choice of $J$ in Algorithm~\ref{alg:MessagePassingUpdate}}
Let $i \in \BV$ be the current factor. For receiving messages, we iterate through all edges $\SN_{\BG}(i)$ in the factor graph and set $J = \{i\}$.
For sending messages, we consider singleton sets $J$, with two exceptions:
When solving~\eqref{eq:UnaryInverseUnaryConstraint}, we set $J = \SX_i$ when $i \in \SV$ is the active factor, and $J = \SX'_{i'}$ when $i' \in \SV'$ is the active one.
For solving~\eqref{eq:FlowUnaryConstraint}, we set $J = \SV$ when the active factor is the assignment factor $f$~\eqref{eq:LinearAssignmentProblem}.

Below we detail solving procedures for~\eqref{eq:ReverseFactorOptimization}  to adjust the messages discussed above with the above choices of $J$.
We always assume that the objective in~\eqref{eq:ReverseFactorOptimization} is $\delta \in \{-1,1\}$.
%
\paragraph{Active factor $i \in \SV \dot{\cup} \SV'$, $J = \{ij\}$:}
\begin{equation}
\label{eq:UnaryToPairwiseMessage}
\phi^*_{(i,ij)}(x_i) = \theta^{\phi}_i(x_i) - \min_{i \in \SX_i} \left\{ \theta^{\phi}_i(x_i) \right\} \quad \forall x_i \in \SX_i\,.
\end{equation}
\paragraph{Active factor $ij \in \SE \dot{\cup} \SE'$, $J = \{i\}$:}
\begin{equation}
\label{eq:PairwiseToUnaryMessage}
\phi^*_{(ij,i)}(x_i) = \min_{x_j \in \SX_{j}} \left\{ \theta^{\phi}_{ij}(x_{ij}) \right\} - \min_{x_{ij} \in \SX_{ij}} \left\{ \theta^{\phi}_{ij}(x_{ij}) \right\}
\quad \forall x_i \in \SX_i\,.
\end{equation}
\paragraph{Active factor $i \in \SV$, $J = \{i'\}, i' \in \SV'$.}
%Let the active factor be $i \in \SV$. For the receive message operation in Algorithm~\ref{alg:AbstractMessagePassing} we have $J = \{i'\}, i' \in \SX_i$ and we compute
\begin{equation}
\label{eq:ReceiveUnaryToInverseUnaryMessage}
\phi^*_{(i,i')} = \min_{x_{i} \in \SX_{i} \backslash \{i'\}} \left\{ \theta^{\phi}_{i}(x_{i}) \right\}\,.
\end{equation}
\paragraph{Active factor $i \in \SV$, $J = \SX_i$}
%For sending messages in Algorithm~\ref{alg:AbstractMessagePassing} we choose $J = \SX_i$ and compute
\begin{equation}
\label{eq:SendUnaryToInverseUnaryMessage}
\phi^*_{(i,i')} = \theta^{\phi}_i(i') - \min_{x_i \in \SX_i} \left\{ \theta^{\phi}_i(x_i) \right\} \quad \forall i' \in \SX_i\,.
\end{equation}
If the active factor is $i' \in \SV'$ , i.e. we solve for $\phi_{(i',i)}$, then either $J = \{i\}$ or $J = \SX'_{i'}$ and everything can be done mutatis mutandis.
%
%\paragraph{(iii) Let $i \in \SV$.}
\paragraph{Active factor $i \in \SV$, $J = \{f\}$} Perform the same operation as in~\eqref{eq:UnaryToPairwiseMessage}, namely
%If the active factor is $i \in \SV$ and $J = \{f\}$, we perform the same operation as in~\eqref{eq:UnaryToPairwiseMessage}, namely
\begin{equation}
\label{eq:UnaryToFlowMessage}
\phi^*_{(i,f)}(x_i) = \theta^{\phi}_i(x_i) -\min_{x_i \in \SX_i} \left\{\theta^{\phi}_i(x_i) \right\} \quad \forall x_i \in \SX_i\,.
\end{equation}
\paragraph{Active factor $f$, $J = \SV$}
%If the active factor is $f$, we choose $J = \SV$. 
Let $\mu_f^*$ be the optimal solution to~\eqref{eq:FactorOptimization}.
Solve
\begin{equation}
\label{eq:LinearAssignmentReparametrizationUpdateProblem}
\begin{array}{lr}
\min_{\mu_f \in \R^{\abs{E}}}  \la \theta^{\phi}_{ass}, \mu_f \ra  & \max_{\pi \in \R^{\abs{\SV}}, ,\pi' \in \R^{\abs{\SV'}}} \la \eins,\pi\ra - \la\eins,\pi',\ra\\
\sum_{j' : (i,j') \in \SE'} \mu_f(i,j') = 1 & \pi(i) \in \R \\
- \sum_{i : (i,j') \in \SE'} \mu_f(i,j') = -1  & \pi'(j') \in \R \\
\mu_f(i,j') \in \left\{ \begin{array}{ll} [1,\infty), & \mu_f^*(i,j') = 0 \\ (-\infty,-1],& \mu_f^*(i,j') = 1 \end{array} \right. 
& \pi(i) - \pi'(j') \leq \theta^{\phi}(i,j')\,, \\
\end{array}
\end{equation}
denote optimal dual variables to~\eqref{eq:LinearAssignmentReparametrizationUpdateProblem} by $\pi^*, \pi'^*$ and set
\begin{equation}
\label{eq:FlowToUnaryMessage}
\phi^*_{(i,f)}(x_i) =  \theta^{\phi}(i,x_i) - \pi^*(i) + \pi'^*(x_i) \,.
\end{equation}
%\begin{remark}
%The optimization problem~\ref{eq:LinearAssignmentReparametrizationUpdateProblem} is similar to the min-marginal update problem described in~\cite{CombinatorialOptimizationMaxProductDuchi}.
%\end{remark}


%\paragraph{(i) Let $i\in \SV \dot{\cup} \SV'$ and $ij \in \SN_{\SG \dot{\cup} \SG'}(i)$.}
%Assume $\mu_i$ is the active factor and $J = \{ij\}$. The adjustment is
%\begin{equation}
%\label{eq:UnaryToPairwiseMessage}
%\phi^*_{(i,ij)}(x_i) = \theta^{\phi}_i(x_i) - \min_{i \in \SX_i} \left\{ \theta^{\phi}_i(x_i) \right\} \quad \forall x_i \in \SX_i\,.
%\end{equation}
%Assume $\mu_{ij}$ is the active factor and $J = \{i\}$. The adjustment is
%\begin{equation}
%\label{eq:PairwiseToUnaryMessage}
%\phi^*_{(ij,i)}(x_i) = \min_{x_j \in \SX_{j}} \left\{ \theta^{\phi}_{ij}(x_{ij}) \right\} - \min_{x_{ij} \in \SX_{ij}} \left\{ \theta^{\phi}_{ij}(x_{ij}) \right\}
%\quad \forall x_i \in \SX_i\,.
%\end{equation}
%\paragraph{(ii) Let $i \in \SV$ and $i' \in \SV'$.}
%Let the active factor be $i \in \SV$. For the receive message operation in Algorithm~\ref{alg:AbstractMessagePassing} we have $J = \{i'\}, i' \in \SX_i$ and we compute
%\begin{equation}
%\label{eq:ReceiveUnaryToInverseUnaryMessage}
%\phi^*_{(i,i')} = \min_{x_{i} \in \SX_{i} \backslash \{i'\}} \left\{ \theta^{\phi}_{i}(x_{i}) \right\}\,.
%\end{equation}
%For sending messages in Algorithm~\ref{alg:AbstractMessagePassing} we choose $J = \SX_i$ and compute
%\begin{equation}
%\label{eq:SendUnaryToInverseUnaryMessage}
%\phi^*_{(i,i')} = \theta^{\phi}_i(i') - \min_{x_i \in \SX_i} \left\{ \theta^{\phi}_i(x_i) \right\} \quad \forall i' \in \SX_i\,.
%\end{equation}
%If the active factor is $i' \in \SV'$ , i.e. we solve for $\phi_{(i',i)}$, then either $J = \{i\}$ or $J = \SX'_{i'}$ and everything can be done mutatis mutandis.
%%
%\paragraph{(iii) Let $i \in \SV$.}
%If the active factor is $i \in \SV$ and $J = \{f\}$, we perform the same operation as in~\eqref{eq:UnaryToPairwiseMessage}, namely
%\begin{equation}
%\label{eq:UnaryToFlowMessage}
%\phi^*_{(i,f)}(x_i) = \theta^{\phi}_i(x_i) -\min_{x_i \in \SX_i} \left\{\theta^{\phi}_i(x_i) \right\} \quad \forall x_i \in \SX_i\,.
%\end{equation}
%If the active factor is $f$, we choose $J = \SV$. 
%Let $\mu_f^*$ be the optimal solution to~\eqref{eq:FactorOptimization}.
%Solve
%\begin{equation}
%\label{eq:LinearAssignmentReparametrizationUpdateProblem}
%\begin{array}{lr}
%\min_{\mu_f \in \R^{\abs{E}}}  \la \theta^{\phi}_{ass}, \mu_f \ra  & \max_{\pi \in \R^{\abs{\SV}}, ,\pi' \in \R^{\abs{\SV'}}} \la \eins,\pi\ra - \la\eins,\pi',\ra\\
%\sum_{j' : (i,j') \in \SE'} \mu_f(i,j') = 1 & \pi(i) \in \R \\
%- \sum_{i : (i,j') \in \SE'} \mu_f(i,j') = -1  & \pi'(j') \in \R \\
%\mu_f(i,j') \in \left\{ \begin{array}{ll} [1,\infty), & \mu_f^*(i,j') = 0 \\ (-\infty,-1],& \mu_f^*(i,j') = 1 \end{array} \right. 
%& \pi(i) - \pi'(j') \leq \theta^{\phi}(i,j')\,, \\
%\end{array}
%\end{equation}
%denote optimal dual variables to~\eqref{eq:LinearAssignmentReparametrizationUpdateProblem} by $\pi^*, \pi'^*$ and set
%\begin{equation}
%\label{eq:FlowToUnaryMessage}
%\phi^*_{(i,f)}(x_i) =  \theta^{\phi}(i,x_i) - \pi^*(i) + \pi'^*(x_i) \,.
%\end{equation}
%
\begin{proposition}
Operations~\eqref{eq:UnaryToPairwiseMessage},~\eqref{eq:PairwiseToUnaryMessage},~\eqref{eq:ReceiveUnaryToInverseUnaryMessage},~\eqref{eq:SendUnaryToInverseUnaryMessage},~\eqref{eq:UnaryToFlowMessage} and~\eqref{eq:FlowToUnaryMessage} all solve~\eqref{eq:ReverseFactorOptimization}.
\end{proposition}





\section{Extensions}
\paragraph{Higher Order}
It is easily possible to extend our approach to higher order graph-matching (called hypergraph-matching in the literature), e.g. with triplet potentials depending on three variables $\theta_{ijk}$.
The corresponding message-passing updates are analoguous to~\eqref{eq:UnaryToPairwiseMessage} and~\eqref{eq:PairwiseToUnaryMessage}.
This also allows to use tighter relaxations based on frustrated cycles~\cite{FrustratedCyclesSontagEtAl}.
\paragraph{Network Flow Constraints}
For the graph-matching problem we have used the linear assignment problem as a factor. 
Analoguously, we could have used a more complex minimum cost flow factor to model other constraints, e.g. 2:1 matching, where at most 2 variables are allowed to match to a given label.
The resulting message-passing update operations would only require changing the underlying graph $\SG_{ass}$ in~\eqref{eq:LinearAssignmentReparametrizationUpdateProblem}.
 % higher order
 % other constraints
 % ...
 

